Network community detection via iterative edge removal in a flocking-like system

We present a network community-detection technique based on properties that emerge from a nature-inspired system of aligning particles. Initially, each vertex is assigned a random-direction unit vector. A nonlinear dynamic law is established so that neighboring vertices try to become aligned with each other. After some time, the system stops and edges that connect the least-aligned pairs of vertices are removed. Then the evolution starts over without the removed edges, and after enough number of removal rounds, each community becomes a connected component. The proposed approach is evaluated using widely-accepted benchmarks and real-world networks. Experimental results reveal that the method is robust and excels on a wide variety of networks. Moreover, for large sparse networks, the edge-removal process runs in quasilinear time, which enables application in large-scale networks.

==> Makefile <==
# Copyright Â© Filipe Neto, Paulo Urio.
# vim: nolist

TARGET = paper.pdf
DEPS_DIR = .deps
BUILD_DIR = build

LATEXMK = latexmk -f -aux-directory=$(BUILD_DIR) -output-directory=$(BUILD_DIR) \
					-recorder -silent -use-make -deps \
					-pdflatex='pdflatex -file-line-error -synctex=1'
WATCH = 0

ifeq ($(WATCH), 1)
	LATEXMK += -pvc
endif

define colorize
	pretty_$1 := sed -e "s/^\([^:]*\)\(:\?\)\([^:]*\):/`tput bold``tput setaf $2`\1`tput sgr0``tput bold``tput setaf 6`\2`tput setaf 2`\3`tput sgr0``tput setaf 6``tput bold`:`tput sgr0`/"
endef

$(eval $(call colorize,box,254))
$(eval $(call colorize,warn,226))
$(eval $(call colorize,ref,214))
$(eval $(call colorize,error,196))
$(eval $(call colorize,check,5))

all: $(BUILD_DIR) $(TARGET)

$(foreach file, $(TARGETS), $(eval -include $(DEPS_DIR)/$(file)P))

$(DEPS_DIR):
	@mkdir $@

$(BUILD_DIR):
	@mkdir $(BUILD_DIR)

%.pdf: %.tex $(DEPS_DIR)
	@test -e .lockmake && echo "Latexmk is already running..." || \
		(touch .lockmake; \
		echo "Running latexmk..."; \
		$(LATEXMK) -pdf -dvi- -ps- -deps-out=$(DEPS_DIR)/$@P $<; \
		rm .lockmake)
	@cd $(BUILD_DIR) && rubber-info -c "biblatex.path .." --boxes ../$< | \
		$(pretty_box)
	@cd $(BUILD_DIR) && rubber-info -c "biblatex.path .." --warnings ../$< | \
		$(pretty_warn) | grep -v "csquotes" || true
	@cd $(BUILD_DIR) && rubber-info -c "biblatex.path .." --refs ../$< | \
		$(pretty_ref)
	@cd $(BUILD_DIR) && rubber-info -c "biblatex.path .." --errors ../$< | \
		$(pretty_error)

clean:
	@echo "Cleaning..."
	@rm -rf .deps
	@find build/ -type f -not -name "*.pdf" -delete

.PHONY: clean

